Knowledge Graphs in Practice: Characterizing their Users, Challenges, and Visualization Opportunities

This study presents insights from interviews with nineteen Knowledge Graph (KG) practitioners who work in both enterprise and academic settings on a wide variety of use cases. Through this study, we identify critical challenges experienced by KG practitioners when creating, exploring, and analyzing KGs that could be alleviated through visualization design. Our findings reveal three major personas among KG practitioners - KG Builders, Analysts, and Consumers - each of whom have their own distinct expertise and needs. We discover that KG Builders would benefit from schema enforcers, while KG Analysts need customizable query builders that provide interim query results. For KG Consumers, we identify a lack of efficacy for node-link diagrams, and the need for tailored domain-specific visualizations to promote KG adoption and comprehension. Lastly, we find that implementing KGs effectively in practice requires both technical and social solutions that are not addressed with current tools, technologies, and collaborative workflows. From the analysis of our interviews, we distill several visualization research directions to improve KG usability, including knowledge cards that balance digestibility and discoverability, timeline views to track temporal changes, interfaces that support organic discovery, and semantic explanations for AI and machine learning predictions.

==> tabulars/kg-definitions.tex <==
% \usepackage{array}

\definecolor{palesilver}{rgb}{0.9, 0.9, 0.9}

\renewcommand\theadalign{bt}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}
% \renewcommand\theadfont{\normalsize\scshape}

% rgb(220,220,220)
% {tabular}{{\raggedleft\arraybackslash}p{0.05\linewidth}>{\raggedleft\arraybackslash}p{0.9\linewidth}}

\resizebox{\textwidth}{!}{
\begin{tabular}[t]{p{0.99\linewidth}}
\toprule

\thead{Knowledge Graph Definitions \& Criteria} \\
\midrule

% A graphical model that represents things or entities and their relationships with each other. It is a graph in the sense that it has vertices and edges. The vertices are the things and the edges are their relationships. This allows for mathematical analysis. \\ \hline
% A directed or undirected graph that shows the relation between entities. Entities can be linked to entities of the same type or different types with different types of relationships.  These relationships are user defined. \\\hline
Consists of nodes and edges, where nodes often represent entities (e.g., objects, subjects, etc.) and edges represent the relationships between the nodes. For example nodes could be movie titles (e.g., Ant Man, Iron Man) and production companies (e.g., Marvel Studios) and an edge connecting these two types of nodes could be ``produced-by". Knowledge graphs can be used to fuse key elements of various data sources to create context that is useful for various information retrieval tasks like question and answering. \\\hline
Helps organize information in a way that can be useful for both humans and machines. Allows for complex relationships to be visualized/processed on. It should be searchable in some sense based on the encoding of it. \\\hline
% A graph that encodes facts and relationships in a structured manner. \\\hline
% Connecting different data sources in a way that adds more meaning than using each data source separately. \\\hline
% An explicit collection of entities and their attributes and relationships. \\\hline
% A set of \{entity - link - entity\} triplets that represents a set of information about some domain. Knowledge graphs tend to be large, although they do not have to be, and often their scale hides complexities in the knowledge that they encode. \\\hline
% A knowledge and data structure for synthesizing relational patterns and dependencies of concepts or data samples. \\\hline
% A heterogeneous graph that represents real world entities. It shows the relationship and connectivity among different entities and types of entities. \\\hline
% A data structure that represents data about the relationships between entities (drugs, genes, diseases, ...) in a way that allows to analyze these relationships or allows to help contextualize experimental results. \\\hline
Maps the relationships between objects (data) and provides information that helps humans and machines understand what the data actually means. A knowledge graph is data plus metadata (or semantic information) linked in a graph. \\\hline
Shows the relationship between entities. More like if you were to put twitter data in a graph database versus looking at a network graph or a purely mathematical graph. So purely that a bunch of nodes are connect does not make a knowledge graph until you give the connections some sort of context or meaning. \\\hline
% Any semantic graph (a graph with labeled edges) and unique nodes is a knowledge graph. \\\hline
A collection of nodes and edges where the nodes correspond to entities and the edges correspond to relationships between entities.  I believe when people refer to knowledge graphs, they refer more to the types of knowledge that are stored, which typically is a set of domain-specific facts that are linked in some way, representing valuable information. \\
% 16  & \add{Fix} \\\hline
% 17  & \add{Fix} \\\hline
% 18  & \add{Fix} \\\hline
% 19  & \add{Fix} \\

% \hline

% PID19 & Staff & Software/Research & Workflows & NA \\

\bottomrule


% \hline

% \rowcolor{palesilver} 
% \strike{PID6}{ PID8}  & SME &  Masters & Pharmacovigilance & (4) Quite familiar     & (3) 1-3x/week & (2) 1-3x/month \\


% \hline
\end{tabular}}

==> tabulars/kg-representations.tex <==
\definecolor{palesilver}{rgb}{0.9, 0.9, 0.9}

\renewcommand\theadalign{bt}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}
% \renewcommand\theadfont{\normalsize\scshape}

% rgb(220,220,220)

\resizebox{\textwidth}{!}{
\begin{tabular}[t]{lll}
\toprule

\textbf{\$ Participants} & 
\textbf{Database or Method} & 
\textbf{Querying Language} \\

\midrule

7  & Neo4J & CYPHER \\
6  & Resource Description Framework & SPARQL \\
4  & Python, NetworkX & (n/a) \\
2  & SQLite3 & SQL \\
1  & Spreadsheet, adjacency matrix & (n/a) \\

% \hline

% \rowcolor{palesilver} 
% \strike{PID6}{ PID8}  & SME &  Masters & Pharmacovigilance & (4) Quite familiar     & (3) 1-3x/week & (2) 1-3x/month \\

\bottomrule
\end{tabular}}


==> tabulars/kg-sizes.tex <==
\definecolor{palesilver}{rgb}{0.9, 0.9, 0.9}

\renewcommand\theadalign{bt}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}

\resizebox{\textwidth}{!}{
\begin{tabular}[t]{lll}
\toprule

\thead{\# Participants} & 
\thead{Estimated Range of Number of Nodes} \\

\hline

8  & Thousands \\
7  & Millions \\
4  & Billions \\

\hline
\end{tabular}}

==> tabulars/visual-tools.tex <==
\definecolor{palesilver}{rgb}{0.9, 0.9, 0.9}

\renewcommand\theadalign{bt}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}

\resizebox{\textwidth}{!}{
\begin{tabular}[t]{ll}
\toprule

\thead{\# Participants} & 
\thead{Graph Visualization Tool, Library, Package} \\

\midrule

7  & Neo4J Bloom \\
5  & Gephi \\
4  & NetworkX (Python) \\
4  & Cytoscape \\
2  & D3 (JavaScript) \\

\hline
6  & No visual tools used \\

\bottomrule
\end{tabular}}
